Nonclassical Measurement Error in the Outcome Variable

We study a semi-/nonparametric regression model with a general form of nonclassical measurement error in the outcome variable. We show equivalence of this model to a generalized regression model. Our main identifying assumptions are a special regressor type restriction and monotonicity in the nonlinear relationship between the observed and unobserved true outcome. Nonparametric identification is then obtained under a normalization of the unknown link function, which is a natural extension of the classical measurement error case. We propose a novel sieve rank estimator for the regression function and establish its rate of convergence. In Monte Carlo simulations, we find that our estimator corrects for biases induced by nonclassical measurement error and provides numerically stable results. We apply our method to analyze belief formation of stock market expectations with survey data from the German Socio-Economic Panel (SOEP) and find evidence for nonclassical measurement error in subjective belief data.

==> Revised Paper/proofs-rates.tex <==

\section{Proofs and Technical Results}\label{Appendix:proofs}
	First, recall that $X=(Z,W)$ and that $g_w=g(\cdot, w)$. 

\begin{proof}[\textsc{Proof of Theorem \ref{thm:ident}.}]
Proof of \eqref{eq:transform}. The exclusion restriction captured in Assumption \ref{A:IV} implies
	\begin{align}\label{Impl.1-3}
	\Ex[Y|X=x] 
	%&= \Ex[\Ex[Y|Y^*, X, W]|X=x, W=w] \\
	&= \Ex[h(Y^*,W)\;|\; Z=z, W=w] \nonumber \\
	&= \Ex[h(g(Z, W)+U, W)\;| \; Z=z, W=w] \nonumber\\
	&= \Ex[h(g(z, W)+U, W) \;|\; W=w],
		\end{align}
	where the last equation is due  to the conditional exogeneity  imposed in Assumption \ref{A:Unobs}. The results follows from strict montonicity of $H(g_w(z), w) =\Ex[h(g(z, W)+U, W) \;|\; W=w]$ in its first argument, which is due to  Assumption \ref{A:Mon} and Assumption \ref{regIdent} (ii). 
	
Proof of \eqref{eq:transform:max}. 	By the law of iterated expectations, the criterion function $Q(\phi,w)=\Ex[Y_1\mathds{1}\{\phi(X_1) > \phi(X_2)\}|W_1=W_2=w]$ can be rewritten as
	\begin{equation*}
	%Q(\phi)&=\Ex[Q(\phi,W)f_W(W)]  \;\;\text{where} 
    Q(\phi,w)=\frac{1}{2}\Ex[H(g(X_1), W_1)\mathds{1}\{ \phi(X_1) > \phi(X_2)\} 
     + H(g(X_2), W_2)\mathds{1}\{ \phi(X_1) < \phi(X_2) \}  \;|\; W_1=W_2=w],
	\end{equation*} 
using $\Ex[Y|X]=H(g(X),W)$ by equation \eqref{eq:transform}. Under Assumption \ref{A:Mon}, we may consider the case that  holds with $h(\cdot,w)$ weakly monotonically increasing, without loss of generality.
%The argument for the decreasing case is analogous.
	Now the function $g_w$ is a maximizer of $Q(\cdot,w)$, which follows by
	\begin{equation*}
	Q(g_w,w) = \frac{1}{2} \Ex[\max\{H(g(X_1),W_1), H(g(X_2),W_2)  \}  \;|\; W_1=W_2=w]
	\end{equation*}
	and using monotonicity of $H$ in its first argument. In particular,  $m \circ g_w$ is a maximizer of $Q(\cdot,w)$ for any strictly increasing function $m$ (here $\circ$ denotes function composition). 
	

%	Let $m(\cdot)$ be some arbitrary strictly increasing function. 
%	This implies that without Assumption \ref{shapecons} the regression function $g_w$ is at best identified up to strictly increasing transformations.
	
	It remains to show that $g_w$ is a unique maximizer up to strictly increasing transformations.
	Specifically, we show that for any function $\widetilde g_w \neq m \circ g_w$ for an arbitrary strictly monotonic transformation $m$ we have that $Q(\widetilde g_w,w) <Q(g_w, w)$. 
%	That is, a function that is not a strictly monotonic transformation of $g_w$ never maximizes the criterion $Q(\cdot,w)$ and thus for an arbitrary $w\in \textsl{supp}(W)$, $g_w$ is identified up to a strictly monotonic transformation which is the main statement of the Theorem. 
	To do so, consider some arbitrary function $\phi \in \mathcal{G}$ that is not a strictly monotonic transformation of $g_w$. Therefore, there exist $z', z''\in\textsl{supp}(Z)$ such that
$g_w (z') < g_w(z'')$ and $	\phi(z') > \phi(z'')$. 
	By \eqref{eq:transform}, $H(\cdot,w)$ is strictly monotonic and it holds for every $w$ that
	\begin{equation*}
	H(g_w(z'),w) < H(g_w(z''),w).
	\end{equation*}
	By continuity of the functions following Assumption \ref{regIdent} (i) the above inequalities hold in neighborhoods $B_1$ around $z'$ and $B_2$ around $z''$, respectively. By Assumption \ref{regIdent} (iii) these neighborhoods have a strictly positive probability measure.
	This implies
	\begin{align*}
	 Q(g_w,w)-Q(\phi ,w)
	 \geq & \frac{1}{2}\Ex[H(g_w(Z_1), W_1) - H(g_w(Z_2), W_2) | Z_1, Z_2 \in B_1 \times B_2, W_1=W_2=w]& \\
	 &  \times \PP(Z_1, Z_2 \in B_1 \times B_2\;|\; W_1=W_2=w) \\
	 >&  0.
	\end{align*}
%with the last inequality following from the strictly positive probability of regions $B_1 \times B_2$.
Thus, $Q(\cdot,w)$ is only maximized by $g_w$ and strictly monotonic transformations of it. Hence, $g_w$ is identified up to a strictly monotonic transformation.
\end{proof}
\begin{proof}[\textsc{Proof of Corollary \ref{coro:ident}.}] 
Under Assumption \ref{shapecons} (i) any candidate regression function $\widetilde g_w(Z)=\widetilde m_w(Z_1)+\widetilde l_w(Z_{-1})$ must satisfy 
\begin{align*}
\widetilde g_w(Z)&= M_w(g_w(Z))=M_w(m_w(Z_1)+l_w(Z_{-1})=\widetilde m_w(Z_1)+\widetilde l_w(Z_{-1})
\end{align*}
for a strictly monotonic function $M_w$. Thus $M_w$ must be linear and $g_w$ is identified up to location and scale transformation. Indeed, given linear and  strictly monotonic transformations, $g_w$ is the only maximizer of $Q(\cdot,w)$. Under Assumption \ref{shapecons} (ii) we have that $g_{w}(z_1)=\Ex[Y|Z=z_1, W=w]$ and $g_{w}(z_2)=\Ex[Y|Z= z_2, W=w]$ and fixing the parameter space to move through both points leads to $g_w$ being the unique maximizer of $Q(\cdot,w)$ over $\mathcal{G}$ and thus $g_w$ is point identified.
\end{proof}


\begin{proof}[\textsc{Proof of Lemma \ref{Lem::AddSep}.}]
	Let $Z_1, Z_2$ be independent copies of $Z$.
	Consider the additive separable case $g(Z_1)=Z_{11} + \widetilde g(Z_{12})$ with bivariate $Z_1=(Z_{11}, Z_{12})$.
	Analogously we denote $\phi(Z_1)=Z_{11} + \widetilde \phi(Z_{12})$. 
	The following holds for the criterion $\mathcal Q$ 
	\begin{align*}
	|\mathcal Q(\phi) |
	=&  \Ex[Y_1(\mathds{1}\{Z_{11} + \widetilde g(Z_{12})  >  g(Z_{2})\} - \Ex[Y_1\mathds{1}\{Z_{11} + \widetilde \phi(Z_{12})  >  \phi(Z_{2})\}]   \\
	=&  \Ex[Y_1 (F_{Z_{21} | Z_{22}}( \phi(Z_{1})- \widetilde \phi(Z_{21})) -F_{Z_{21} | Z_{22}}( g(Z_{1})- \widetilde g(Z_{21})) )]    ,
	\end{align*}
	as $g$ is the maximizer of $\mathcal{Q}$ and with the second equation due to the law of iterated expectation.
	Using a second-order Taylor decomposition with directional derivatives yields for all $\phi$ in a neighborhood around $g$
	\begin{align*}
	|\mathcal Q(\phi) | = &  Q_g(\phi -g)  + \underbrace{\Ex[Y_1 f^{''}_{Z_{21} | Z_{22}}(\xi)(\widetilde\phi(Z_{12}) - \widetilde g(Z_{12}) +    \widetilde g(Z_{22}) - \widetilde \phi (Z_{22}) )^3 ]}_{=R},
\end{align*}
where $\xi$ is some intermediate variable\footnote{More precisely $\xi=g(Z_{1})- \widetilde g(Z_{22})+ s[\phi(Z_1)-\widetilde \phi(Z_{21}) + \widetilde g(Z_{21})-g(Z_{1})]$ for some $s\in (0,1)$.} and $Q_g$ denotes the directional derivative of $\mathcal Q$ at $g$ which is given by
\begin{align*}
 Q_g(\phi-g)= &\Ex[Y_1 f'_{Z_{21} | Z_{22}}(g(Z_{1})- \widetilde g(Z_{21}))(\widetilde\phi(Z_{12}) - \widetilde g(Z_{12}) +    \widetilde g(Z_{22}) - \widetilde \phi (Z_{22}) )^2 ].
	\end{align*}
	 Applying the Cauchy-Schwarz inequality to $Q_g(\phi-g)$ shows that $Q_g$ is weaker than the $L^2$-norm.
	Further, the remainder term $R$ satisfies
	\begin{equation*}
	|R| \leq \Ex \left[\left|\frac{f^{''}_{Z_{21} | Z_{22}}(\xi)}{f'_{Z_{21} | Z_{22}}(g(Z_{1})- \widetilde g(Z_{21}))}(\widetilde\phi(Z_{12}) - \widetilde g(Z_{12}) +    \widetilde g(Z_{22}) - \widetilde \phi (Z_{22}) )\right| \right] \cdot Q_g(\phi-g)
	\end{equation*}
	and thus the tangential cone condition in Assumption \ref{A:Rate} (iv) is satisfied if the first factor on the right hand side is bounded between 0 and 1. The lower bound holds directly and the upper bound is easily satisfied if the $\delta-$ neighborhood around $g$ is chosen sufficiently small and derivatives of the density are bounded away from zero and infinity, as is condition.
\end{proof}
For the proof of the next results, we require some additional notation to deal with the Hoeffding decomposition of U-statistics, specific function spaces and their respective envelope functions.

We introduce the empirical criterion $\mathcal Q_n(\phi)$ that can be denoted as
\begin{align*}
 \mathcal Q_n(\phi) &  = \frac{2}{n(n-1)}\sum_{1 \leq i < j \leq n} \Gamma(S_i, S_j, \phi)  
%\Gamma(S_i, S_j, \phi)&:=K_h(W_i-w)K_h(W_j-w)Y_i[\mathds{1}(\phi(Z_i)>\phi(Z_j))- \mathds{1}(g_w(Z_i)>g_w(Z_j))] 
\end{align*}
where $S_i=(Y_i, Z_i)$ and which is a second order U-statistic with kernel
\begin{align*}
\Gamma(S_i, S_j, \phi) =  Y_i\big(\mathds{1}\{\phi(Z_i)>\phi(Z_j)\}- \mathds{1}\{g(Z_i)>g(Z_j)\}\big)
\end{align*}
indexed by $\phi \in \mathcal{G}_K$ making it a second-order U-process. Note that $\mathcal{Q}_n$ is centered here which does not affect the optimization. Using the kernel notation, the criterion function $\mathcal{Q}$ given in \eqref{def:crit:centered} satisfies $\mathcal{Q}(\phi)= \Ex[\Gamma(S_i, S_j, \phi)]$.

For the asymptotic analysis we make use of the Hoeffding decomposition of a U-statistic (see e.g. \cite{vanVaart98})
\begin{align}\label{Hoeffding}
\mathcal{Q}_n(\phi) =   \mathcal{Q}(\phi) + \nu_n(\phi) +  \xi_n(\phi) 
\end{align}
with short hand notations
\begin{align*}
\nu_n(\phi) &:= \frac{1}{n}\sum_{i=1}^{n} \nu(S_i, \phi),\\
\nu(S_i, \phi) &:=  \Ex[\Gamma(S_i, S_j, \phi)| S_i] + \Ex[\Gamma(S_j, S_i, \phi)|S_i]- 2\Ex[\Gamma(S_i, S_j,\phi)],  \\
\xi_n(\phi) &:= \frac{2}{n(n-1)} \sum_{1 \leq i < j \leq n} \xi(S_i, S_j, \phi), \\
\xi(S_i, S_j, \phi) &:= \Gamma(S_i,S_j, \phi) - \Ex[\Gamma(S_i,S_j, \phi)| S_i] - \Ex[\Gamma(S_i, S_j, \phi)|S_j] + \Ex[\Gamma(S_i, S_j,\phi)].
\end{align*}
This decomposition is frequently deviced in the rank estimation literature to obtain asymptotic results, see e.g. \cite{sherman93}. The first summand in the decomposition is a smooth function of the parameter $\phi$, $\nu_n$ is an empirical process and $\xi_n$ a degenerate U-process, both indexed by the function space $\mathcal{G}_K$.

Further, we define the function classes $\mathcal{F}_{\nu,K}=\{ \nu(\cdot, \phi): \phi \in \mathcal{G}^\delta_K\}$ and  $\mathcal{F}_{\xi,K}=\{ \xi(\cdot, \cdot, \phi): \phi \in \mathcal{G}_K^\delta\}$. Let $\overline F_\nu$ and $\overline F_\xi$ denote respective envelope functions .
The envelope function is defined as any function satisfying $|\nu(\cdot,\phi)|\leq \overline F_\nu(\cdot)$.
In this setting, $\overline F_\nu(S_i) = |Y_i| + 3 \Ex[|Y_i|]$, since
\begin{align*}
|\nu(S_i, \phi)| = &| Y_i\Ex[\mathds{1}\{\phi(Z_i) > \phi(Z_j)\} - \mathds{1}\{g(Z_i) > g(Z_j)\}|Z_i]\\
& +\Ex[Y_j \left(\mathds{1}\{\phi(Z_j) > \phi(Z_i)\} - \mathds{1}\{g(Z_j) > g(Z_i)\} \right)|Z_i] \\
& - 2\Ex[ Y_i \left(\mathds{1}\{\phi(Z_i) > \phi(Z_j)\} - \mathds{1}\{g(Z_i) > g(Z_j)\} \right) ]| \\
\leq & |Y_i| + 3\Ex[|Y_i|],
\end{align*}
where $\mynorm*{\overline F_\nu}_{L^2(S)} \leq \sqrt{4\Ex[Y^2]} =: C_\nu$. 
In addition we have $\overline F_{\xi}(S_i, S_j)=2|Y_i|+2\Ex[|Y_i|]$ as
\begin{align*}
|\xi(S_i, S_j, \phi)| = & | Y_i(\mathds{1}\{\phi(Z_i) > \phi(Z_j)\} - \mathds{1}\{g(Z_i) > g(Z_j)\}) \\
-&  Y_i\Ex[\mathds{1}\{\phi(Z_i) > \phi(Z_j)\} - \mathds{1}\{g(Z_i) > g(Z_j)\} |Z_i ] \\
-&  \Ex[Y_i(\mathds{1}\{\phi(Z_i) > \phi(Z_j)\} - \mathds{1}\{g(Z_i) > g(Z_j)\}) |Z_j ] \\
+&  \Ex[Y_i(\mathds{1}\{\phi(Z_i) > \phi(Z_j)\} - \mathds{1}\{g(Z_i) > g(Z_j)\})] |
\end{align*}
and $\mynorm*{\overline F}_{L^2(S)} \leq \sqrt{12\Ex[Y^2]} =: C_\eta$. By Assumption \ref{A:Rate} (iii) we have $C_\nu, C_\eta< \infty$.
Ultimately, we define the bracketing integral $J_{[]}$ of the space $\mathcal{F}_{\nu, K}$  
\begin{align*}
J_{[]}(1,\mathcal{F}_{\nu,K},  L^2(S))= \int_{0}^{1} \sqrt{1+ \log N_{[]} (\epsilon \cdot \mynorm*{\overline F_\nu}_{L^2(S)},\mathcal{F}_{\nu,K}, L^2(S)) } d\epsilon.
\end{align*}
and analogously for $\mathcal{F}_{\xi, K}$.

\begin{proof}[\textsc{Proof of Theorem \ref{thm::rate}.}]
We begin by noting that consistency of $\widehat{g}$ in the $L^2$-norm follows from Lemma \ref{App::Lemma2}.
Due to the consistency result in  Lemma \ref{App::Lemma2}, we may restrict the function spaces to a local neighborhood around $g$, i.e. we define the space $\mathcal{G}^\delta_K = \{\phi \in \mathcal{G}_K : \mynorm*{\phi-g}_{L^2(Z)}< \delta\}$ and assume that $\widehat g \in \mathcal{G}^\delta_K $. Further we introduce the space $\mathcal{G}^{\delta,r_n}_K =\{ \phi \in \mathcal{G}^\delta_K :  Q_g(\phi-g) > Mr_n  \}$ where $M>0$.
It holds that
\begin{align*}
 \PP\big( Q_g(\widehat{g}-g) &\geq Mr_n\big)
\leq  \PP \left( \sup_{\phi\in\mathcal{G}^{\delta,r_n}_K} \mathcal Q_n(\phi) \geq  \mathcal Q_n(\Pi_Kg) \right)\\
\leq & \PP \left( \sup_{\phi\in\mathcal{G}^{\delta,r_n}_K} \mathcal Q(\phi) + \nu_n(\phi) + \xi_n ( \phi) \ \geq \mathcal Q(\Pi_Kg) + \nu_n(\Pi_Kg) + \xi_n (\Pi_Kg) \right),
\end{align*}
by applying the Hoeffding decomposition (\ref{Hoeffding}).
Due to Assumption \ref{A:Rate} (iv) we have local equivalence of $|\mathcal Q(\cdot)|$ and $Q_g(\cdot)$. Since $\mathcal Q(\cdot)$ is negative and thus $|\mathcal Q(\cdot)|=-\mathcal Q (\cdot)$ it follows that
{\small \begin{flalign*}
  \PP \big( Q_g(\widehat{g}-g) \geq Mr_n \big) &\leq  \PP \left( \sup_{\phi\in\mathcal{G}^{\delta,r_n}_K} \Big(\mathcal Q(\phi) +  \nu_n(\phi)-\nu_n(\Pi_Kg) + \xi_n (\phi) -\xi_n (\Pi_Kg)) \Big)\geq - \eta Q_g(\Pi_Kg-g) \right) &\\
\leq & \PP \left(\sup_{\phi\in\mathcal{G}^{\delta,r_n}_K} \Big(\nu_n(\phi)-\nu_n(\Pi_Kg) + \xi_n (\phi) -\xi_n (\Pi_Kg)+\eta Q_g(\Pi_Kg-g) \Big)\geq \inf_{\phi\in\mathcal{G}^{\delta,r_n}_K} |\mathcal Q(\phi)| \right) \\
\leq & \PP \left(\sup_{\phi\in\mathcal{G}^\delta_K} \nu_n(\phi)-\nu_n(\Pi_Kg)  + \sup_{\phi\in\mathcal{G}^\delta_K} \xi_n (\phi) -\xi_n (\Pi_Kg) + \eta Q_g(\Pi_Kg-g) \geq C_2Mr_n  \right),
\end{flalign*}}%
%\begin{align*}
%& \PP \left( \mynorm*{\widehat g-g} \geq Mr_n \right) \\
% \leq & \PP \left( \sup_{\mathcal{G}^\delta_K: \mynorm*{\phi-g} > Mr_n} \mathcal Q_n(\phi) \geq  \mathcal Q_n(\Pi_Kg) \right) \\
%\leq & \PP \left( \sup_{\mathcal{G}^\delta_K: \mynorm*{\phi-g} > Mr_n} \mathcal Q(\phi) + P_n v(\phi) + U_n \xi ( \phi) \ \geq \mathcal Q(\Pi_Kg) + P_n v(\Pi_Kg) + U_n \xi (\Pi_Kg) \right) \\
%\leq & \PP \left( \sup_{\mathcal{G}^\delta_K: \mynorm*{\phi-g} > Mr_n} \mathcal Q(\phi) + P_n (v(\phi)-v(\Pi_Kg)) + U_n (\xi (\phi) -\xi (\Pi_Kg)) \geq -C_1 ||\Pi_Kg-g|| \right) \\
%\leq & \PP \left(\sup_{\mathcal{G}^\delta_K: \mynorm*{\phi-g} > Mr_n} P_n (v(\phi)-v(\Pi_Kg)) + U_n (\xi (\phi) -\xi (\Pi_Kg)) \geq C_2Mr_n -C_1 ||\Pi_Kg-g|| \right) \\
%\leq & \PP \left(\sup_{\mathcal{G}_K} P_n ( v(\phi)-v(\Pi_Kg))  + \sup_{\mathcal{G}_K} U_n (\xi (\phi) -\xi (\Pi_Kg)) + C_1 ||\Pi_Kg-g|| \geq C_2Mr_n  \right) 
%\end{align*}
where it remains to study the asymptotic behavior of each summand in the last line separately. 
Note that both summands on the left hand-side are positive, hence if $\sup_{\mathcal{G}^\delta_K}  \nu_n(\phi)$ is bounded in probability so is $ \nu_n(\Pi_Kg)$ and similarly for $\xi_n$.

First we study the asymptotic behavior of the empirical process part $\sup_{\phi \in\mathcal G^\delta_K}  \nu_n(\phi)$. Recall the definition $\mathcal{F}_{\nu,K}=\{ \nu(\cdot, \phi): \phi \in \mathcal{G}^\delta_K\}$ with envelope $\overline F_\nu$. 
By applying the last display of Theorem 2.14.2 of \cite{Vaart2000} we can conclude that 
\begin{align*}
\Ex \Big| \sup_{\phi \in\mathcal G^\delta_K} \nu_n(\phi)\Big| = \Ex \Big|\sup_{\nu \in \mathcal{F}_{\nu,K}} \frac{1}{n}\sum_{i=1}^{n} \nu(S_i) \Big| \leq J_{[]}(1,\mathcal{F}_{\nu,K}, L^2(S))\cdot \mynorm*{\overline F_\nu}_{L^2(S)}\cdot n^{-1/2}
\end{align*}
where $\mynorm*{\overline F_\nu}_{L^2(S)} \leq \mynorm*{\overline F_\nu}_{L_\infty(S)} \leq C_\nu< \infty$. 
By Lemma \ref{App::Lemma1} (i) and (ii) we have
\begin{align*}
\log N_{[]} (\epsilon \cdot \mynorm*{\overline F_\nu}_{L_\infty(S)}, \mathcal{F}_{\nu,K},  L_\infty(S)) \leq c_0 K \log(1/\epsilon \cdot C_\nu^{-1} )
\end{align*}
and ultimately we obtain $J_{[]}(1, \mathcal{F}_{\nu,K}, L_\infty(S))=O(\sqrt{K})$ and by Markov's inequality $\sup_{\phi \in \mathcal{G}^\delta_K} \nu_n(\phi) = O_p(\sqrt{K/n})$.

It remains to analyze the convergence rate of the degenerate U-process $\sup_{\phi \in \mathcal{G}^\delta_K} \xi_n(\phi)$. Similar to Lemma A.1 in \cite{ClemLugosi08} we can make use of the following equality for second-order U-statistics 
\begin{align}\label{ClemLug}
\frac{1}{n(n-1)} \sum_{i \neq j} \xi(S_i, S_j, \phi) = \frac{1}{n!} \sum_{\pi} \frac{1}{\lfloor n/2 \rfloor} \sum_{i=1}^{\lfloor n/2 \rfloor} \xi(S_i, S_{\lfloor n/2 \rfloor + i}, \phi)
\end{align}
where $\pi$ is short-hand for all permutations of  $\{1,\dots, n\}$. Then applying the triangle inequality to (\ref{ClemLug}) leads to 
\begin{equation}\label{UStatIneq}
\Ex \left[ \Big| \sup_{\phi \in \mathcal{G}^\delta_K}  \frac{1}{n(n-1)} \sum_{i \neq j} \xi(S_i, S_j, \phi) \Big| \right] \leq \Ex \left[ \Big |\sup_{\phi \in \mathcal{G}^\delta_K}  \frac{1}{\lfloor n/2 \rfloor} \sum_{i=1}^{\lfloor n/2 \rfloor} \xi(S_i, S_{\lfloor n/2 \rfloor + i}, \phi) \Big | \right]
\end{equation}
from which we can conclude that for obtaining the convergence rate of the degenerate U-process on the left-hand side of (\ref{UStatIneq}) it is sufficient to analyze the convergence rate of an empirical process with kernel $\xi$ indexed by the function $\mathcal{G}^\delta_K$.

The kernel $\xi$ contains non-smooth indicator functions so we cannot apply the exact same reasoning we used earlier to derive a bound for $\nu_n$, as $\xi(S_i, S_j, \phi)$ is not continuous in $\phi$.  
However we can use the fact that $\xi(\cdot, \cdot, \phi)$ belongs to a VC- subgraph family and we can thus derive the complexity bound in Lemma \ref{App::Lemma1} (iii).

Recall the definition $\mathcal{F}_{\xi, K}=\{ \xi(\cdot, \cdot, \phi): \phi \in \mathcal{G}_K^\delta\}$ and the associated envelope function $\overline F_\xi$.
Now we apply Theorem 2.14.1 of \cite{Vaart2000}
\begin{equation*}
\Ex \left[ \Big |\sup_{\phi \in \mathcal{G}^\delta_K}  \frac{1}{\lfloor n/2 \rfloor} \sum_{i=1}^{\lfloor n/2 \rfloor} \xi(S_i, S_{\lfloor n/2 \rfloor + i}, \phi) \Big | \right] \leq J_{[]}(1,\mathcal F_{\xi, K}, L^2(S))\mynorm*{\overline F_\xi}_{L^2(S)}\lfloor (n/2)\rfloor^{-1/2}
\end{equation*}
Applying Lemma \ref{App::Lemma1} (iii) we obtain the bound
\begin{align*}
J_{[]}(1, \mathcal{F}_{\xi, K}, L^2(S)) \leq  \int_{0}^{1} \sqrt{1+ c_1+c_2K\log(1/\epsilon) }d\epsilon = O(\sqrt{K})
\end{align*}
and by Markov's inequality that $\sup_{\phi \in \mathcal{G}^\delta_K}  \xi_n(\phi)=O_p(\sqrt{K/n})$.
%It suffices to find a bound for $sup_{\phi \in \mathcal{G}}  U_n \xi(\phi)$. 
%We can apply Corollary 8 in \cite{sherman94} to establish that $sup_{\phi \in \mathcal{G}}  U_n \xi(\phi)=o_p(1)$. The euclidean property of the function class $\{ \xi(\cdot, \cdot, \phi): \phi \in \mathcal{G}\}$ follows *from Assumption \ref{A:Rate} (iv).
Finally, we can conclude that
\begin{equation*}
\PP \left( Q_g(\widehat g-g) \geq Mr_n \right)
%\leq \PP \left(O_p(\sqrt{K/n})  + O_p(\sqrt{K/n}) + O(Q_g(\Pi_Kg-g)) \geq C_2Mr_n \right).
\leq \PP \left(\sup_{\phi \in \mathcal{G}^\delta_K}  \nu_n(\phi)  + \sup_{\phi \in \mathcal{G}^\delta_K}  \xi_n(\phi) + Q_g(\Pi_Kg-g) \geq C_2Mr_n \right).
\end{equation*}
with $\sup_{\phi \in \mathcal{G}^\delta_K}  \nu_n(\phi)=O_p(\sqrt{K/n})$ and $\sup_{\phi \in \mathcal{G}^\delta_K}  \xi_n(\phi)=O_p(\sqrt{K/n})$.
Consequently,  choosing $r_n=\max\{ \sqrt{K/n},Q_g(\Pi_Kg-g)\}$ we see that the right hand side probability converges to zero as $M \to \infty$. Thus $Q_g(\widehat{g}-g) =O_p(r_n)$.  By the definition of the sieve measure of ill-posedness $\tau_K$ we obtain
\begin{equation*}
\mynorm*{\widehat{g} - g}_{L^2(Z)}  \leq \tau_K Q_g(\widehat{g} - g) 
                            \leq \tau_K O_p\left( \max\{ \sqrt{K/n}, Q_g(\Pi_Kg-g)\} \right) = O_p\left( \tau_K \sqrt{K/n}, \mynorm*{\Pi_Kg-g}_{L^2(Z)}\right) 
\end{equation*}
%\begin{align*}
%\mynorm*{\widehat{g} - g}_{L^2(Z)} & \leq \mynorm*{\widehat{g} - \Pi_Kg}_{L^2(Z)} + \mynorm*{\Pi_Kg-g}_{L^2(Z)} \\
%& \leq \tau_K Q_g(\widehat{g} - \Pi_Kg) + \mynorm*{\Pi_Kg-g}_{L^2(Z)} \\
%& = O_p( \tau_K r_n) + \mynorm*{\Pi_Kg-g}_{L^2(Z)}
%\end{align*}
which concludes the proof. 
\end{proof}

\begin{lem}\label{App::Lemma1}
Under Assumption \ref{A:Rate} it holds that\\
(i) $\sup_{\mynorm*{\phi-g}_\infty \leq \delta} |\nu(S_i,\phi)|\leq M_1(S_i)\cdot \delta$ with $\Ex[M_1(S_i)] < \infty $, 	\\
(ii) $\log N_{[]} (\epsilon,\mathcal{F}_{\nu,K}, L_\infty(S)) \leq  c_0K\log(1/\epsilon) $ for some positive constant $c_0$, \\
(iii)  $\log N(\epsilon,\mathcal{F}_{\xi,K}, L^2(S)) \leq c_1+c_2K\log(1/\epsilon)$, for positive constants $c_1,c_2$.
\end{lem} 
\begin{proof}[\textsc{Proof of Lemma \ref{App::Lemma1}.}] 
Proof of part (i). It holds that
\begin{align*}
\nu(S_i, \phi) = & Y_i\Ex[\mathds{1}\{\phi(Z_i) > \phi(Z_j)\} - \mathds{1}\{g(Z_i) > g(Z_j)\}|Z_i]\\
& +\Ex[Y_j \left(\mathds{1}\{\phi(Z_j) > \phi(Z_i)\} - \mathds{1}\{g(Z_j) > g(Z_i)\} \right)|Z_i] \\
& - 2\Ex[ Y_i \left(\mathds{1}\{\phi(Z_i) > \phi(Z_j)\} - \mathds{1}\{g(Z_i) > g(Z_j)\} \right) ]
\end{align*}
We make use of the fact that as $ \mynorm*{\phi-g}_\infty \leq \delta$ and thus $g(z) - \delta \leq \phi(z)\leq g(z)+\delta$ for any $z$ in the support of $Z$. Following \cite{ChenShen2003} (p. 1599-1600) we have that
\begin{equation*}
\sup_{\mynorm*{\phi-g}_\infty \leq \delta}|\mathds{1}\{\phi(Z_j) < \phi(Z_i) \} - \mathds{1}\{g(Z_j) < g(Z_i)\} |
\leq  |\mathds{1}\{g(Z_j) < \phi(Z_i)+\delta \} - \mathds{1}\{g(Z_j) < g(Z_i) - \delta \} | 
\end{equation*}
and thus 
\begin{align*}
|\nu(S_i, \phi)| \leq  &  |Y_i|\cdot |F_{g(Z)}( \phi(Z_i)+\delta) - F_{g(Z)}( g(Z_i) -\delta) |  \\
                      & + |\Ex[Y_i|Z_i]|\cdot |F_{g(Z)}( \phi(Z_i)+\delta) - F_{g(Z)}( g(Z_i) -\delta) | \\
                      &+ |\Ex[Y_i]|\cdot \Ex[|F_{g(Z)}( \phi(Z_i)+\delta) - F_{g(Z)}( g(Z_i) -\delta) |  ] \\
                 \leq & (|Y_i| + |\Ex[Y_i|Z_i]| + |\Ex[Y_i]|) \cdot 3\delta    
\end{align*}
where the last inequality follows from Assumption \ref{A:Rate} (v), the Lipschitz continuity for the cdf of $g(Z)$. Define $M_1(S_i) = |Y_i| + |\Ex[Y_i|Z_i]| + |\Ex[Y_i]| $. From Assumption \ref{A:Rate} (iii) follows that $\Ex[M_1(S_i)]< \infty$ which concludes the argument.

We continue with the proof of  part (ii).
By Lemma \ref{App::Lemma1} (i) we have
\begin{align*}
\log N_{[]} (\epsilon, \mathcal{F}_{\nu,K},  L_\infty(S)) \leq \log N_{[]} (\epsilon, \mathcal{G}_K,  L_\infty(Z)) \leq cK \log(1/\epsilon)
\end{align*} 
where both inequalities are due to \cite{Chen07} (pp. 5595 and 5601).

We conclude with the proof of part (iii). We make use of the decomposition $\xi(S_i, S_j, \phi)  = \xi_1(S_i, S_j, \phi) + \xi_2(S_i, S_j, \phi)$ where $\xi_1(S_i, S_j, \phi)  = \Gamma(S_i,S_j, \phi) $ and 
\begin{align*}
\xi_2(S_i, S_j, \phi)  = - \Ex[\Gamma(S_i,S_j, \phi)| S_i] - \Ex[\Gamma(S_i, S_j, \phi)|S_j] + \Ex[\Gamma(S_i, S_j,\phi)].
\end{align*}
Following for instance \cite[Lemma 16]{NolanPollard} we conclude
\begin{align*}
\log N(\epsilon,\mathcal{F}_{\xi,K}, L^2(S)) \leq \log N(\epsilon,\mathcal{F}_{\xi_1,K}, L^2(S)) + \log N(\epsilon,\mathcal{F}_{\xi_2,K}, L^2(S)).
\end{align*}
Similar to the proof of part (ii) of Lemma \ref{App::Lemma1} we obtain
$\log N(\epsilon,\mathcal{F}_{\xi_2,K}, L^2(S))\leq cK \log(1/\epsilon) $ for some constant $c$.
Below, we follow Chapter 5 of \cite{sherman93} to establish that $ \mathcal{F}_{\xi_1,K}$ belongs to a VC-subgraph class.
To this end define the subgraph 
\begin{flalign*}
\text{subgraph}\left(\xi_1(\cdot, \cdot, \phi) \right)=&\{(s_i,s_j,t) \in \textsl{supp}(S)^2\times \mathbb{R}: 0<t< y_i[\mathds{1}\{\phi(z_i) > \phi(z_j) \} - \mathds{1}\{g(z_i) < g(z_j)\} ] \}& \\
 = &\{y_i > 0\}\{\phi(z_i)- \phi(z_j) > 0  \}\{t > 0 \}\{t < \overline F_{\xi_1}(z_i, z_j) \} \{g(z_i)-g(z_j)  < 0 \} \\
 &\cup \{y_i < 0\}\{\phi(z_i)- \phi(z_j) < 0  \}\{t > 0 \}\{t < \overline F_{\xi,1}(z_i, z_j) \} \{g(z_i)-g(z_j)  > 0 \}
\end{flalign*}
and introduce the function 
\begin{align*}
m(t, s_1, s_2; \gamma_1, \gamma_2, \pi_1, \pi_2):=\gamma_1t+ \gamma_2y_1+(g(z_1), p^K(z_2))'\pi_1 + (g(z_2), p^K(z_2))'\pi_2 
\end{align*} 
with the associated function space
\begin{align*}
\mathcal{M}=\{m(\cdot, \cdot, \cdot; \gamma_1, \gamma_2, \pi_1, \pi_2): \gamma_1\in \mathbb{R}, \gamma_2\in \mathbb{R}, \pi_1\in \mathbb{R}^{K+1}, \pi_2\in \mathbb{R}^{K+1}\}.
\end{align*} 
Note that $\mathcal{M}$ is a finite vector space of dimension $2(K+2)$ and the subgraph can be written as
\begin{align}\label{subgraph_decomp}
\text{subgraph}\left(\xi_1(\cdot, \cdot, \phi) \right) & =\bigcup_{i=1}^{10} \{m_i > 0\}
\end{align}
with functions $m_i \in \mathcal{M}$ for any $i=1,\dots, 10$. 
Following e.g. Lemma 2.4 and 2.5 in \cite{pakespollard89} it can be established that $\text{subgraph}\left(\xi_1(\cdot, \cdot, \phi) \right)$ belongs to a VC-class of sets and thus the space $\mathcal{F}_{\xi_1}$ is a VC-class of functions.
To bound the complexity of the space we require the VC-index of $\mathcal{F}_{\xi_1}$ which we denote as $V(\mathcal{F}_{\xi_1})=V(\text{subgraph}(\xi_1))$.
 
From \cite[ Lemma 18]{Pollard84} it follows that $V(\{m_i > 0\})\leq 2(K+2)$. Applying in \cite[Theorem 1.1]{vdVaart_VCdim} to (\ref{subgraph_decomp}) then leads to $V(\text{subgraph}(\xi_1))\lesssim 2(K+2)$, so the VC-index of the space $\mathcal{F}_{\xi_1}$ increases with the same order as the sieve dimension $K$. 
Now applying \cite[Theorem 2.6.7]{vanVaart98} yields
\begin{align*}
\log N(\epsilon,\mathcal{F}_{\xi_1,K}, L^2(S)) &\leq \log( C\cdot V(\mathcal{F}_{\xi_1}) (16e)^{V(\mathcal{F}_{\xi_1})}(1/\epsilon)^{2V(\mathcal{F}_{\xi_1})-2}) \\
& = \log(C)+ \log(2(K+2)) + 2(K+2)\log(16e)  + 2(K+2)\log(1/\epsilon)
\end{align*}
and together with $\log N(\epsilon,\mathcal{F}_{\xi_2,K}, L^2(S))\leq cK \log(1/\epsilon) $ the stated result follows. 
\end{proof}

\begin{lem}\label{App::Lemma2}
	Under Assumptions \ref{A:IV}--\ref{A:Rate} it holds that $\mynorm{\widehat g - g}_{L^2(Z)} = o_p(1)$. 
\end{lem} 
\begin{proof}[\textsc{Proof of Lemma \ref{App::Lemma2}.}] 
		We need to check the conditions in Lemma A.2 of \cite{ChenPouzo12}. 
		In their notation $\overline Q_n = \mathcal{Q}$ and
		\begin{align*}
		g_0(k, n, \epsilon)=\inf_{\phi \in \mathcal{G}_K: \mynorm{\phi- g}_{L^2(Z)} \geq \epsilon} |\mathcal{Q}(\phi)|
		\end{align*}
		Their condition a is thus satisfied and $g_0(n,k, \epsilon) > 0 $ by the identification result in Theorem \ref{thm:ident}. 
	    Condition b holds by Assumption \ref{A:Rate} (ii) and the fact that for large enough $K$ the following holds
       \begin{align*}
       |\mathcal Q(\Pi_Kg) -\mathcal Q(g)| \lesssim Q_g(\Pi_Kg - g) \lesssim \tau^{-1}_K \mynorm{\Pi_Kg -g}_{L^2(Z)},
       \end{align*} 
	    and thus  $\mathcal Q(\Pi_Kg) - \mathcal Q(g) = o(1)$.
	    Next, Condition c is implicitly assumed to hold and it remains to check condition d which translates as 
		\begin{align*}
		\frac{\max\{ |\mathcal Q(\Pi_Kg) - \mathcal Q(g)| , \sup_{\phi \in \mathcal{G}_K} |\mathcal{Q}_n(\phi) -\mathcal Q(\phi)|    \}}{g_0(n,k, \epsilon)} =o(1).
		\end{align*}
		Analogous to the empirical process result from (\ref{ClemLug}) and (\ref{UStatIneq}) and the subsequent proceedings, it holds that		$\sup_{\phi \in \mathcal{G}_K} |\mathcal{Q}_n(\phi) -\mathcal Q(\phi)| \lesssim \sqrt{K/n}$.
				Then ultimately consider that for any $\epsilon>0$ there is some $\epsilon^*>0$ that is  sufficiently small such that the local equivalence relation in Assumption \ref{A:Rate} (iv) is valid and we can conclude  
		{\small \begin{equation*}
		g_0(k,n, \epsilon) = \inf_{\mathcal{G}_K: \mynorm{\phi -g}_{L^2(Z)}\geq \epsilon} |\mathcal{Q}(\phi)|  \geq \inf_{\mathcal{G}_K: \mynorm{\phi -g}_{L^2(Z)}\geq \epsilon^*} Q_g(\phi-g) \geq \inf_{\mathcal{G}_K: \mynorm{\phi -g}_{L^2(Z)}\geq \epsilon^*} \tau^{-1}_K \mynorm{\phi -g}_{L^2(Z)}  \geq \tau^{-1}_K \epsilon^*.
		\end{equation*}}
	In summary we require that 
		\begin{equation*}
		\max\{ |\mathcal Q(\Pi_Kg) - \mathcal Q(g)| , \sup_{\phi \in \mathcal{G}_K} |\mathcal{Q}_n(\phi) -\mathcal Q(\phi)|    \} \big/ g_0(n,k, \epsilon) 
		\lesssim \tau_K\max\{ \sqrt{K/n} , \tau^{-1}_K \mynorm{\phi -g}_{L^2(Z)}    \} = o(1),
		\end{equation*}
		which follows from the rate restriction in Assumption \ref{A:Rate} (vi).
\end{proof}
